EFSMT: A Logical Framework for Cyber-Physical Systems

The design of cyber-physical systems is challenging in that it includes the analysis and synthesis of distributed and embedded real-time systems for controlling, often in a nonlinear way, the environment. We address this challenge with EFSMT, the exists-forall quantified first-order fragment of propositional combinations over constraints (including nonlinear arithmetic), as the logical framework and foundation for analyzing and synthesizing cyber-physical systems. We demonstrate the expressiveness of EFSMT by reducing a number of pivotal verification and synthesis problems to EFSMT. Exemplary problems in this paper include synthesis for robust control via BIBO stability, Lyapunov coefficient finding for nonlinear control systems, distributed priority synthesis for orchestrating system components, and synthesis for hybrid control systems. We are also proposing an algorithm for solving EFSMT problems based on the interplay between two SMT solvers for respectively solving universally and existentially quantified problems. This algorithms builds on commonly used techniques in modern SMT solvers, and generalizes them to quantifier reasoning by counterexample-guided constraint strengthening. The EFSMT solver uses Bernstein polynomials for solving nonlinear arithmetic constraints.

==> Preliminaries_CH.tex <==
\section{Preliminaries}\label{sec.prelim}

Let $\overline{x}$, $\overline{y}$ be a vector of $m$ and $n$ disjoint
variables. The general form of \emph{exists-forall problems} is
represented in Eq.~\ref{eq.forall.general}, where $[\overline{l_{x}},
\overline{u_{x}}] = [l_{x_1}, u_{x_1}]\times\ldots\times [l_{x_m},
u_{x_m}] \subseteq \mathbb{Q}^{m}$ and $[\overline{l_{y}},
\overline{u_{y}}] = [l_{y_1}, u_{y_1}]\times\ldots \times[l_{y_n},
u_{y_n}]\subseteq \mathbb{Q}^{n}$ is the \emph{domain} for
$\overline{x}$ and $\overline{y}$. $\phi(\overline{x}, \overline{y})$
is a quantifier-free formula that involves variables from
$\overline{x}$ and $\overline{y}$ of \textsf{boolean},
\textsf{integer}, or \textsf{real}. We assume that the formula is well-formed,
i.e. it evaluates to either \textsf{true} or \textsf{false} provided
that all variables are assigned. Therefore, we do not require all variables to have the same type.
%\remark{type}{Should all variables have the same type?}.

\vspace{-2mm}
\begin{equation}\label{eq.forall.general}
\exists \overline{x} \in [\overline{l_{x}}, \overline{u_{x}}] \; \forall \overline{y} \in [\overline{l_{y}}, \overline{u_{y}}]:
\phi(\overline{x}, \overline{y})
\end{equation}
%\vspace{1mm}

$\phi(\overline{x}, \overline{y})$ is composed from a propositional combination of
\begin{inparaenum}[(a)]
\item boolean formula,
\item linear arithmetic for integer variables, and
\item linear and nonlinear polynomial constraints for real
  variables.
\end{inparaenum}This combination enables the framework to model
discrete control in the computation unit (e.g., CPU),
physical constraints in the environment, and constraints of device
models. Specially, we find the use of Eq.~\ref{eq.forall.assume.guarantee} with the condition that
(1) $\rho_{jp}, \varphi_j$ are polynomials over real variables in $\overline{x}, \overline{y}$ and
(2) $\textsf{op}_{jp}, \textsf{op}_{j}\in \{>,\geq,<,\leq\}$
particularly useful to be applied in cyber-physical systems.

\vspace{-2mm}
\begin{multline}\label{eq.forall.assume.guarantee}
\exists \overline{x} \in [\overline{l_{x}}, \overline{u_{x}}] \; \forall \overline{y} \in [\overline{l_{y}}, \overline{u_{y}}]: \\
\bigwedge^k_{j=1}  ((\bigwedge^{q}_{p=1} \rho_{jp}(\overline{x}, \overline{y})\,\textsf{op}_{jp}\,d_{jp})
\rightarrow \varphi_j(\overline{x}, \overline{y})\,\textsf{op}_j\,e_j)
\end{multline}

Intuitively, $\rho_{jp}(\overline{x},
\overline{y})\,\textsf{op}_{jp}\,d_{jp}$ states the \emph{assumptions} of a particular scenario (indexed by
$j$) for the environment, and $\varphi_j(\overline{x},
\overline{y})\,\textsf{op}_j\,e_j$ formulates the corresponding
\emph{guarantee} provided by the system under operation.

Modern SMT solvers support other established theories (i.e. a set of
formulas closed under logical validity) such as the theory of arrays, lists and sets.
We do not consider these theories in \textsf{ExForSMT}, since they are
related to the verification of programs in high-level languages such
as C or Java. Also, \textsf{ExForSMT} can not handle nonlinear polynomial
constraints that are not built from finitely many monomials of
$\overline{x}, \overline{y}$ (e.g. $\sin, \tan, \lg$). Still, one can
often rewrite these functions as polynomials of $\overline{x},
\overline{y}$ and $z$, where $z$ is a universal variable with bounded
real domain that gives a conservative error estimate.

%Modern SMT solvers support other established theories\footnote{A theory is a set of formulas $T$ that is closed under logical validity.} such as the theory of arrays, lists or sets. These theories are not considered in \textsf{ExForSMT}, as they are more related to the verification of programs in high-level languages such as C or Java. Also, \textsf{ExForSMT} is not designed to handle nonlinear polynomial constraints that are not built from finitely many monomials of $\overline{x}, \overline{y}$ (examples include $\sin, \tan, \lg$). Still,  these functions can very often be rewritten as polynomials of $\overline{x}, \overline{y}$ and $z$, where $z$ is a universal variable with bounded real domain to give a conservative estimate on errors.

\vspace{1mm}
\noindent \textbf{(Example)} The following constraint $(\exists x \in [-30,30]\cap\mathbb{R})~(\forall y \in [-30, 30]\cap\mathbb{R}): (0<y<10) \rightarrow (y-2x<7)$ is an exists-forall problem targeted by \textsf{ExForSMT}. The interpretation domain of each variable is provided in the quantification (although $\mathbb{R}$ is usually omitted).


